Topology and Routing Problems: The Circular Frame

In this work, we solve the problem of finding non-intersecting paths between points on a plane with a new approach by borrowing ideas from geometric topology, in particular, from the study of polygonal schema in mathematics. We use a topological transformation on the 2-dimensional planar routing environment that simplifies the routing problem into a problem of connecting points on a circle with straight line segments that do not intersect in the interior of the circle. These points are either the points that need to be connected by non-intersecting paths or special `reference' points that parametrize the topology of the original environment prior to the transformation. When all the necessary points on the circle are fully connected, the transformation is reversed such that the line segments combine to become the non-intersecting paths that connect the start and end points in the original environment. We interpret the transformed environment in which the routing problem is solved as a new data structure where any routing problem can be solved efficiently. We perform experiments and show that the routing time and success rate of the new routing algorithm outperforms the ones for the A*-algorithm.

==> pref.tex <==

\newcommand{\todo}[1]{{\bf ?????!!!! #1 ?????!!!!}\marginpar{$\Longleftarrow$}}
\newcommand{\tocite}{{[!CITE!]}\marginpar{$\Longleftarrow\Longleftarrow!!!$}}
\newcommand{\tocheck}{{[!CHECK!]}\marginpar{$\Longleftarrow\Longleftarrow!!!$}}
\newcommand{\towrite}{{[WRITING...]}\marginpar{$\Longleftarrow\Longleftarrow!!!$}}

\newcommand{\bcomment}[1]{\noindent\textcolor{blue}{(#1)}}
\newcommand{\rcomment}[1]{\noindent\textcolor{red}{(#1)}}
\newcommand{\gcomment}[1]{\noindent\textcolor{green}{(#1)}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\beql}[1]{\begin{equation}\label{#1}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\beal}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}
\newcommand{\eref}[1]{(\ref{#1})}
\newcommand{\sref}[1]{\S\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\pa}{\partial}
\newcommand{\oline}{\overline}
\newcommand{\bvec}{\left(\ba{c}}
\newcommand{\evec}{\ea\right)}
\newcommand{\bvset}[1]{\left\{\ba{#1}}
\newcommand{\evset}{\ea\right\}}
\newcommand{\fref}[1]{Figure \ref{#1}}
\newcommand{\btab}[1]{\begin{tabular}{#1}}
\newcommand{\etab}{\end{tabular}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\master}{\mathcal{F}^\flat}
\newcommand{\irrmaster}{{}^{\text{Irr}}\mathcal{F}^\flat}
\newcommand{\mesonic}{\mathcal{M}^{mes}}

\def \Red {\pdfsetcolor{0 1 1 0}}
\def \Green {\pdfsetcolor{1 0 1 0}}
\def \Blue {\pdfsetcolor{1 1 0 0}}
\def \Black {\pdfsetcolor{0 0 0 1}}

\newcommand{\BC}{\mathbb{C}}
\newcommand{\BR}{\mathbb{R}}
\newcommand{\BZ}{\mathbb{Z}}
%\newcommand{\comment}[1]{}
\newcommand{\CF}{{\cal F}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CW}{{\cal W}}
\newcommand{\CN}{{\cal N}}
\newcommand{\CB}{{\cal B}}
\newcommand{\IP}{\mathbb{P}}
\newcommand{\IC}{\mathbb{C}}
\newcommand{\vev}[1]{\langle #1 \rangle}
\def\tQ{\widetilde{Q}}
\def\tB{\widetilde{B}}

\newcommand{\ud}{\mathrm{d}}
\newcommand{\bull}{$\bullet\ $}
\newcommand{\CP}{\mathbb P}

\newcommand{\PE}{\mathrm{PE}}
%\newcommand{\PE}[1]{\mathrm{PE}\left[#1\right]}
\newcommand{\PL}{\mathrm{PL}}
%\newcommand{\PL}[1]{\mathrm{PL}\left[#1\right]}

\newcommand{\mqcd}{\CM_{(N_f,N_c)}}

\newtheorem{theorem}{\bf Theorem}
\def\thetheorem{\thesection.\arabic{theorem}}
\newtheorem{conjecture}[theorem]{\bf Conjecture}
\newtheorem{observation}[theorem]{\bf Observation}
\newtheorem{lemma}[theorem]{\bf Lemma}

\def\theequation{\thesection.\arabic{equation}}
\newcommand{\setall}{\setcounter{equation}{0}
        \setcounter{theorem}{0}}
\newcommand{\setequation}{\setcounter{equation}{0}}


\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\qed}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}
      
      
\newcommand{\cM}{{\cal M}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cZ}{{\cal Z}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cX}{{\cal X}}
\newcommand{\IA}{\mathbb{A}}
%\newcommand{\IP}{\mathbb{P}}
\newcommand{\IQ}{\mathbb{Q}}
\newcommand{\IH}{\mathbb{H}}
\newcommand{\IN}{\mathbb{N}}
\newcommand{\IR}{\mathbb{R}}
%\newcommand{\IC}{\mathbb{C}}
\newcommand{\IF}{\mathbb{F}}
\newcommand{\IV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\IZ}{\mathbb{Z}}
\newcommand{\re}{{\rm~Re}}
\newcommand{\im}{{\rm~Im}}

\newcommand{\td}{{\rm Td}}      


\newcommand{\V}{\mathcal{V}}
\newcommand{\wV}{\widetilde{\mathcal{V}}}
\newcommand{\wmaster}{\widetilde{\master}}
\newcommand{\Tr}{\text{Tr}}
\newcommand{\ra}{\rightarrow}
\newcommand{\cp}{\mathbb{C}\mathbb{P}}
%\definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
%\definecolor{forestgreen}{rgb}{0.13, 0.55, 0.13}

